Object DGCNN: 3D Object Detection using Dynamic Graphs

3D object detection often involves complicated training and testing pipelines, which require substantial domain knowledge about individual datasets. Inspired by recent non-maximum suppression-free 2D object detection models, we propose a 3D object detection architecture on point clouds. Our method models 3D object detection as message passing on a dynamic graph, generalizing the DGCNN framework to predict a set of objects. In our construction, we remove the necessity of post-processing via object confidence aggregation or non-maximum suppression. To facilitate object detection from sparse point clouds, we also propose a set-to-set distillation approach customized to 3D detection. This approach aligns the outputs of the teacher model and the student model in a permutation-invariant fashion, significantly simplifying knowledge distillation for the 3D detection task. Our method achieves state-of-the-art performance on autonomous driving benchmarks. We also provide abundant analysis of the detection model and distillation framework.

==> section/broader_impact.tex <==
\section{Broader Impact}
The goal of this paper is to improve the object detection pipeline, which is crucial for the safety of autonomous driving systems. We hope this work can contribute to bringing self driving cars (or autonomous systems more broadly) to reality sooner, to reduce traffic accidents, and to increase productivity. Future work to improve applicability in this domain might consider challenges of \emph{explainability}, which currently elude popular object detection models.
